PolyReal: A Benchmark for Real-World Polymer Science Workflows

Multimodal Large Language Models (MLLMs) excel in general domains but struggle with complex, real-world science. We posit that polymer science, an interdisciplinary field spanning chemistry, physics, biology, and engineering, is an ideal high-stakes testbed due to its diverse multimodal data. Yet, existing benchmarks related to polymer science largely overlook real-world workflows, limiting their practical utility and failing to systematically evaluate MLLMs across the full, practice-grounded lifecycle of experimentation. We introduce PolyReal, a novel multimodal benchmark grounded in real-world scientific practices to evaluate MLLMs on the full lifecycle of polymer experimentation. It covers five critical capabilities: (1) foundational knowledge application; (2) lab safety analysis; (3) experiment mechanism reasoning; (4) raw data extraction; and (5) performance & application exploration. Our evaluation of leading MLLMs on PolyReal reveals a capability imbalance. While models perform well on knowledge-intensive reasoning (e.g., Experiment Mechanism Reasoning), they drop sharply on practice-based tasks (e.g., Lab Safety Analysis and Raw Data Extraction). This exposes a severe gap between abstract scientific knowledge and its practical, context-dependent application, showing that these real-world tasks remain challenging for MLLMs. Thus, PolyReal helps address this evaluation gap and provides a practical benchmark for assessing AI systems in real-world scientific workflows.

==> tables/table2.tex <==
% \begin{table}[t!]
% \centering
% \caption{Performance comparison on polymer science benchmarks. F1-scores are reported. SA: Spectroscopy Analysis, RDA: Raw Data Analysis, PLS: Polymer Lab Safety.}
% \label{tab:polymer_results_f1_only} % 我修改了标签以反映F1-only
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{lrrr}
% \toprule
% \textbf{Model} & \textbf{SA (F1)} & \textbf{RDA (F1)} & \textbf{PLS (F1)} \\
% \midrule
% \textbf{Qwen\_Qwen2.5-VL-72B-Instruct} & 0.064 & 0.058 & 0.144 \\
% \textbf{Qwen\_Qwen3-VL-235B-A22B-Thinking} & 0.097 & 0.183 & 0.347 \\
% \textbf{Qwen\_Qwen3-VL-32B-Thinking} & 0.181 & 0.150 & 0.230 \\
% \textbf{claude-sonnet-4-5-20250929-thinking} & 0.275 & 0.151 & 0.317 \\
% \textbf{deepseek-ai\_deepseek-vl2} & 0.000 & 0.022 & 0.036 \\
% \textbf{deepseek-r1} & 0.245 & 0.265 & 0.136 \\
% \textbf{gemini-2.0-flash-thinking-exp} & 0.116 & 0.113 & 0.267 \\
% \textbf{gemini-2.5-flash} & 0.232 & 0.233 & 0.369 \\
% \textbf{gemini-2.5-pro} & 0.490 & 0.187 & 0.366 \\
% \textbf{gpt-4o} & 0.015 & 0.158 & 0.117 \\
% \textbf{gpt-4o-mini} & 0.022 & 0.037 & 0.078 \\
% \textbf{gpt-5} & 0.353 & 0.192 & 0.373 \\
% \textbf{grok-4} & 0.149 & 0.093 & 0.224 \\
% \textbf{intern-s1} & 0.057 & 0.062 & 0.249 \\
% \textbf{o3} & 0.298 & 0.251 & 0.412 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

\begin{table}[t!]
\centering
\caption{Performance comparison on \textit{PolyReal} benchmarks. F1-scores are reported. SA: Spectroscopy Analysis, RDA: Raw Data Analysis, PLS: Polymer Lab Safety.}
\label{tab:polymer_results_f1_only} % 我修改了标签以反映F1-only
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lrrr}
\toprule
\textbf{Model} & \textbf{SA} & \textbf{RDA} & \textbf{PLS} \\
\midrule
\textbf{Qwen2.5-VL-72B-Instruct} & 0.064 & 0.058 & 0.144 \\
\textbf{Qwen3-VL-235B-A22B-Thinking} & 0.097 & 0.183 & 0.347 \\
\textbf{Qwen3-VL-32B-Thinking} & 0.181 & 0.150 & 0.230 \\
\textbf{Claude-Sonnet-4.5-Thinking} & 0.275 & 0.151 & 0.317 \\
\textbf{DeepSeek-VL2} & 0.000 & 0.022 & 0.036 \\
\textbf{DeepSeek-R1} & 0.245 & 0.265 & 0.136 \\
\textbf{Gemini-2.0-Flash-Thinking} & 0.116 & 0.113 & 0.267 \\
\textbf{Gemini-2.5-Flash} & 0.232 & 0.233 & 0.369 \\
\textbf{Gemini-2.5-Pro} & 0.490 & 0.187 & 0.366 \\
\textbf{GPT-4o} & 0.015 & 0.158 & 0.117 \\
\textbf{GPT-4o-mini} & 0.022 & 0.037 & 0.078 \\
\textbf{GPT-5} & 0.353 & 0.192 & 0.373 \\
\textbf{Grok-4} & 0.149 & 0.093 & 0.224 \\
\textbf{Intern-S1} & 0.057 & 0.062 & 0.249 \\
\textbf{o3} & 0.298 & 0.251 & 0.412 \\
\bottomrule
\end{tabular}%
}
\end{table}
